On the Determinant of One-Dimensional Elliptic Boundary Value Problems

We discuss the $\zeta-$regularized determinant of elliptic boundary value problems on a line segment. Our framework is applicable for separated and non-separated boundary conditions.

==> rrdummy.tex <==
%
% CMR font family for math symbols by Ingo Eichenseher
%
\font\tenrr=cmbx10  scaled \magstep1
\font\sevenrr=cmbx7 scaled \magstep1
\font\fiverr=cmbx5 scaled \magstep1

\newfam\rrfam
\textfont\rrfam=\tenrr
\scriptfont\rrfam=\sevenrr
\scriptscriptfont\rrfam=\fiverr

\def\A{{\fam\rrfam A}}
\def\B{{\fam\rrfam B}}
\def\C{{\fam\rrfam C}}
\def\D{{\fam\rrfam D}}
\def\E{{\fam\rrfam E}}
\def\F{{\fam\rrfam F}}
\def\G{{\fam\rrfam G}}
\def\H{{\fam\rrfam H}}
\def\I{{\fam\rrfam I}}
\def\J{{\fam\rrfam J}}
\def\K{{\fam\rrfam K}}
\def\L{{\fam\rrfam L}}
\def\M{{\fam\rrfam M}}
\def\N{{\fam\rrfam N}}
\def\O{{\fam\rrfam O}}
\def\P{{\fam\rrfam P}}
\def\Q{{\fam\rrfam Q}}
\def\R{{\fam\rrfam R}}
%\def\S{{\fam\rrfam S}}
\def\T{{\fam\rrfam T}}
\def\U{{\fam\rrfam U}}
\def\V{{\fam\rrfam V}}
\def\W{{\fam\rrfam W}}
\def\X{{\fam\rrfam X}}
\def\Y{{\fam\rrfam Y}}
\def\Z{{\fam\rrfam Z}}
\def\one{{\fam\rrfam 1}}

